A Case for CXL-Centric Server Processors

The memory system is a major performance determinant for server processors. Ever-growing core counts and datasets demand higher bandwidth and capacity as well as lower latency from the memory system. To keep up with growing demands, DDR--the dominant processor interface to memory over the past two decades--has offered higher bandwidth with every generation. However, because each parallel DDR interface requires a large number of on-chip pins, the processor's memory bandwidth is ultimately restrained by its pin-count, which is a scarce resource. With limited bandwidth, multiple memory requests typically contend for each memory channel, resulting in significant queuing delays that often overshadow DRAM's service time and degrade performance. We present CoaXiaL, a server design that overcomes memory bandwidth limitations by replacing \textit{all} DDR interfaces to the processor with the more pin-efficient CXL interface. The widespread adoption and industrial momentum of CXL makes such a transition possible, offering $4\times$ higher bandwidth per pin compared to DDR at a modest latency overhead. We demonstrate that, for a broad range of workloads, CXL's latency premium is more than offset by its higher bandwidth. As CoaXiaL distributes memory requests across more channels, it drastically reduces queuing delays and thereby both the average value and variance of memory access latency. Our evaluation with a variety of workloads shows that CoaXiaL improves the performance of manycore throughput-oriented servers by $1.52\times$ on average and by up to $3\times$.

==> extensions.tex <==
\section{Extensions}
\label{sec:extensions}


\ad{We may drop this section. (+1 Anish)}

This work focuses on the extra memory bandwidth ultimately translating to performance gain decreasing queuing delay and tail memory access latency. However, we believe there are other ways to utilize or translate the abundance of memory bandwidth to performance even in low utilized systems. One potential example is more aggressive prefetching. Prefetching generates more memory traffic that may not be useful, so there is potential risk of hurting the performance by increasing the memory bandwidth utilization. \TheName decreases this risk, as contribution to bandwidth utilization from the prefetcher is proportionally smaller. To demonstrate our case we conduct a quick experiment with next N line prefetcher, where we increase N to model more aggressive prefetching, on a scaled down 8 core system. For memory configuration, we compare DDR, 2X CXL and 4X CXL both with 30ns added latency. We give 1 memory controller for DDR. For workload we chose pagerank.
We observe that DDR starts losing performance even at prefetching one line. 2X CXL has a significant performance gain from no prefetching to 1 line, but starts losing performance at 2 lines. 4X CXL gains performance up to 4 lines, starts losing at 8 lines. This demonstrates the the abundance in bandwidth allows more aggressive prefetching without significant penalty. Unfortunately, with the naive next line prefetcher, we don't see notable gain beyond 1 line even for 4X CXL. However, with the state of art prefetchers, \TheName will enable them to prefetch more candidate lines. Of course, prefetcher still has to be used with caution as even \TheName could still reach high bandwidth utilization. Prefetching can also result in cache pollution, but in this experiment we didn't see a noticeable effect.

Another design extension from a different angle is a multi-socket system that mitigates NUMA effect. Unlike DDR, CXL can cover up to 1 meter of physical distance without repeater. This lets each socket to connect to all the CXL memory controllers. Also, it is worth noting that CXL inherently decreases the need due to its capacity advantage against DDR. We further imagine a shared memory pool CXL memory attached to multiple processing nodes as their main memory, which would decrease the amount of memory needed. However there are schools of design challenges, including managing and allocating memory to nodes, as is the case even with disaggregated shared supplementary memory pool.



==> implementation.tex <==


\section{Implementation}
\label{sec:implementation}



==> intro.tex <==
\section{Introduction}
\label{sec:intro}






Multi-core designs and, more recently, chiplet processor architectures have been delivering performance gains despite the end of Dennard scaling and the slowdown of Moore's law in the past two decades. 
At the same time, as the data consumed by processors is increasing exponentially, technological breakthroughs have enabled higher-capacity memory with new media like non-volatile RAM or via remote memory access over fast networks (e.g., RDMA). 
A common technological trade-off with higher-capacity memory is significantly slower memory access latency and aggregate bandwidth compared to the DDR-based main memory. 
As a result, servers continue to predominantly rely on DDR-attached memory for performance while optionally retaining a slower memory tier like NVRAM or remote DRAM for capacity expansion.

The emerging Compute Express Link (CXL) standard bridges the performance gap between low-bandwidth, high-capacity memory and DDR-based main memory. 
By attaching DRAM modules over the widely deployed high-bandwidth PCI Express (PCIe) bus, CXL vastly improves memory capacity and bandwidth, while retaining DDR-like characteristics at a modest access latency overhead. 
Consequently, there has recently been much interest in architecting CXL-based memory systems that enable memory pooling and capacity expansion \cite{ahn:enabling,gouk:direct,li:pond,marouf:tpp}. %

CXL owes its high bandwidth to the underlying PCIe-based serial interface, which currently delivers about $4\times$ higher bandwidth per processor pin compared to the parallel DDR interface, with technological roadmaps projecting this gap to grow further. 
Hence, by repurposing the processor's DDR-allocated pins to CXL, it is possible to quadruple the available memory bandwidth.
However, the higher bandwidth comes at the cost of memory access latency overhead, expected to be as low as 25--30ns \cite{cxl-3.0, plda:cxl-latency}, although higher in initial implementations and systems that multiplex CXL memory devices across multiple processors. 
Low access latency is a key requirement for high-performance memory,  which is why CXL's latency overhead has biased the research so far to treat the technology exclusively as a memory \textit{expansion} technique rather than a \textit{replacement} of local DDR-attached memory.

However, we observe that the overall latency of memory access in a loaded memory system is dominated by the queuing delay at the memory controller, which arbitrates access to the DDR channel. 
Modern servers feature between 4 and 16 cores per memory channel, resulting in contention and significant queuing delays even before a request can be launched over the memory bus. 
While these queuing delays can be mitigated by provisioning more memory channels, doing so requires more processor pins, which are a scarce resource. %
Given rigid pin constraints, CXL's bandwidth-per-pin advantage can be leveraged to unlock significant bandwidth and performance gains by rethinking memory systems to be CXL-centric rather than DDR-centric. %

In this paper, we make the key observation that the bandwidth boost attainable with  CXL drastically reduces memory access queuing delays, which largely dictate the effective access latency of loaded memory systems. 
Driven by this insight, we argue that \textit{a memory system attached to the processor {entirely} over CXL} is a key enabler for scalable high-performance server processors that deploy memory-intensive workloads. %
Our proposed server design, dubbed \TheName, replaces all of the processor's direct DDR interfaces with CXL.

\ifvariance
Our evaluation shows that \TheName delivers average performance gains of $\mytodo{}\times$ for typical memory-intensive server workloads like graph and data analytics, transaction processing, and machine learning, due to two main reasons. 
First, a loaded memory system's effective latency is often dominated by the impact of queuing effects and therefore significantly differs from the unloaded system's latency, as we demonstrate in \cref{sec:motivation:queuing-impact}. 

Second, while a memory system's average memory access latency is an important performance determinant, the variance in accessing memory also plays a critical role.
Even the most aggressive cores with wide reorder buffers inevitably stall whenever a memory access misses in the cache hierarchy. 
However, due to the memory-level parallelism  
 (MLP) exhibited by typical memory-intensive applications, the core usually has groups of several concurrently outstanding memory accesses. 
The long latency of the slowest memory access in this group can end up stalling the reorder buffer much more compared to the average access.
We demonstrate the impact of memory access latency variance in \cref{sec:motivation:variance}.
\else
Our evaluation shows that \TheName delivers average performance gains of $\mytodo{}\times$ for typical memory-intensive server workloads like graph and data analytics, transaction processing, and machine learning.
A loaded memory system's effective latency is often dominated by the impact of queuing effects and therefore significantly differs from the unloaded system's latency, as we demonstrate in \cref{sec:motivation:queuing-impact}. 
\fi

By evaluating \TheName with a range of representative server and desktop workloads, we highlight how CXL-based memory system's unique characteristics (i.e., increased bandwidth and higher unloaded latency) positively impact performance of processors whose memory system is typically loaded.
Our analysis presents simple but often overlooked facts about memory system behavior and its impact on overall performance, offering strong motivation for a radical change in memory system design that departs from two decades of DDR and enables scalable high-performance server architectures.
In particular, a memory system that offers higher parallelism reduces queuing effects, which in turn results in lower average latency and variance, even if its unloaded access latency is higher compared to existing systems.
We argue that CXL-based memory systems offer exactly this design trade-off, which is favorable for loaded server processors handling memory-intensive applications.


In summary, we make the following contributions:
\begin{itemize}[noitemsep,topsep=0pt,leftmargin=*]

    \item We make the radical proposal of using high-bandwidth CXL as a \textit{complete replacement} of pin-inefficient DDR interfaces on server processors, showcasing a ground-breaking shift that disrupts decades-long memory system design practices. %
    \ifvariance
    \item We show how our design, \TheName, reduces queuing delays and variance of memory accesses, highlighting that unloaded latency and average memory access time alone are incomplete metrics for assessing server memory systems.  
    \else
    \item We show that, despite its higher unloaded memory access latency, \TheName reduces the effective memory access time in typical scenarios where the memory system is loaded.
    \fi
    \item We demonstrate the promise of \TheName with a study of both server and desktop \mytodo{?} applications for a variety of CXL bandwidth and latency design points that are likely in the near future. 
    \item We identify limitations imposed on CXL by the current PCIe standard, and highlight opportunities a hypothetical revised standard could leverage for \mytodo{$\times$} additional speedup.
\end{itemize}

\smallskip
\noindent\textit{Paper outline:}
\cref{sec:motivation} describes the technological trends enabling the replacement of DDR with CXL in server processors.
\cref{sec:queuing-effect} highlights how critical a memory system's queuing delays and access latency variance are, both of which a CXL-based memory system can mitigate, and \cref{sec:design} provides an overview of our proposed \TheName server design.
We outline the methodology to evaluate \TheName against a DDR-based system in \cref{sec:method} and analyze performance results in \cref{sec:eval}.
We discuss related work in \cref{sec:related} and conclude in \cref{sec:conclusion}.


==> result-checklist.tex <==

\newcommand{\missing}{\noindent{\color{red} {\textit{missing}}}}
\newcommand{\done}{\noindent{\color{green} {\textit{done}}}}


\begin{table*}[]
\centering
\begin{tabular}{|c|c|c|c|cc|cc|}
\hline
                                    &           & baseline & core sensitivity & \multicolumn{2}{c|}{BW sensitivity}    & \multicolumn{2}{c|}{latency sensitivity}     \\ \hline
App group                           & App       & 128c/4x  & 64c/4x           & \multicolumn{1}{c|}{128c/2x} & 128c/8x & \multicolumn{1}{c|}{128c/+10ns} & 128c/+50ns \\ \hline
\multirow{6}{*}{\textbf{Tailbench}} & img-dnn   & \done    &                  & \multicolumn{1}{c|}{}        &         & \multicolumn{1}{c|}{}           &            \\ \cline{2-8} 
                                    & moses     & \done    & \done            & \multicolumn{1}{c|}{\done}   & \done   & \multicolumn{1}{c|}{\done}      & \done      \\ \cline{2-8} 
                                    & sphinx    & \done    &                  & \multicolumn{1}{c|}{}        &         & \multicolumn{1}{c|}{}           &            \\ \cline{2-8} 
                                    & masstree  & \done    &                  & \multicolumn{1}{c|}{}        &         & \multicolumn{1}{c|}{}           &            \\ \cline{2-8} 
                                    & xapian    & \done    &                  & \multicolumn{1}{c|}{}        &         & \multicolumn{1}{c|}{}           &            \\ \cline{2-8} 
                                    & shore     & \missing &                  & \multicolumn{1}{c|}{}        &         & \multicolumn{1}{c|}{}           &            \\ \hline
\textbf{KVS}                        & MICA      & \done    &                  & \multicolumn{1}{c|}{}        &         & \multicolumn{1}{c|}{}           &            \\ \hline
\multirow{6}{*}{\textbf{GAP}}       & pagerank  &  &                  & \multicolumn{1}{c|}{}        &         & \multicolumn{1}{c|}{}           &            \\ \cline{2-8} 
                                    & sssp      &     &                  & \multicolumn{1}{c|}{}        &         & \multicolumn{1}{c|}{}           &            \\ \cline{2-8} 
                                    & tc        &  &                  & \multicolumn{1}{c|}{}        &         & \multicolumn{1}{c|}{}           &            \\ \cline{2-8} 
                                    & cc        &  \done    &                  & \multicolumn{1}{c|}{}        &         & \multicolumn{1}{c|}{}           &            \\ \cline{2-8} 
                                    & bfs       &     &                  & \multicolumn{1}{c|}{}        &         & \multicolumn{1}{c|}{}           &            \\ \cline{2-8} 
                                    & bc        &     &                  & \multicolumn{1}{c|}{}        &         & \multicolumn{1}{c|}{}           &            \\ \hline
\multirow{8}{*}{\textbf{SPEC}}      & mcf       &          & \done            & \multicolumn{1}{c|}{}        &         & \multicolumn{1}{c|}{}           &            \\ \cline{2-8} 
                                    & omnetpp   &          &             & \multicolumn{1}{c|}{}        &         & \multicolumn{1}{c|}{}           &            \\ \cline{2-8} 
                                    & xalancbmk &          &             & \multicolumn{1}{c|}{}        &         & \multicolumn{1}{c|}{}           &            \\ \cline{2-8} 
                                    & blender   &          &             & \multicolumn{1}{c|}{}        &         & \multicolumn{1}{c|}{}           &            \\ \cline{2-8} 
                                    & lbm       &          &             & \multicolumn{1}{c|}{}        &         & \multicolumn{1}{c|}{}           &            \\ \cline{2-8} 
                                    &  deepsjeng    &     \done     &             & \multicolumn{1}{c|}{}        &         & \multicolumn{1}{c|}{}           &            \\ \cline{2-8} 
                                    & perlbench &  \done   &             & \multicolumn{1}{c|}{}        &         & \multicolumn{1}{c|}{}           &            \\ \cline{2-8} 
                                    &           &          &             & \multicolumn{1}{c|}{}        &         & \multicolumn{1}{c|}{}           &            \\ \hline
\textbf{TPC-H}                      & MonetDB   & \done    &                  & \multicolumn{1}{c|}{}        &         & \multicolumn{1}{c|}{}           &            \\ \hline
\end{tabular}
\caption{Status of different applications used in evaluation.}
\end{table*}

==> tbl-request-lat.tex <==


\begin{table}[]
\centering
\begin{tabular}{|c|cc|c|}
\hline
\multirow{2}{*}{workload} & \multicolumn{2}{c|}{ application p99 latency (\microsecond)} & \multirow{2}{*}{Difference} \\ \cline{2-3} 
                          & \multicolumn{1}{c|}{\mbox{\hspace{4mm}}DDR\mbox{\hspace{4mm}}}     & CXL  &    \\ \hline
                  moses    & \multicolumn{1}{c|}{12.6}        &   4.90   &  $-61\%$\\ \hline
                imgdnn   & \multicolumn{1}{c|}{4.41}        &   1.56    & $-65\%$\\ \hline
                masstree   & \multicolumn{1}{c|}{0.36}       &   0.13 & $-64\%$\\ \hline
                xapian    & \multicolumn{1}{c|}{8.02}        &  7.99    &  $\sim0\%$ \\ \hline
\end{tabular}
\caption{Application request service time tail latency. 
}
\label{table:req_lat}
\end{table}




==> tbl_apps_old.tex <==
\begin{table}[!b]
\begin{center}
\begin{footnotesize}
\def\arraystretch{1.2}  
\vspace{-5mm}
\caption{Workload Summary. \ac{to update}}
\label{table:apps}
\begin{tabular}{ | l | c | c | l | c | c | }
\hline
\multicolumn{3}{|c|}{Server applications} & \multicolumn{3}{c|}{Desktop applications (SPEC)}\\
\hline
Application & IPC & LLC MPKI & Application & IPC & LLC MPKI\\ 
\hline \hline
moses & 0.35 & 26 & lbm & 0.36 & 22 \\  
\hline
masstree & 0.37 & 27  &  omnetpp & 0.67 & 14 \\  
\hline
img-dnn & 0.37 & 37 & parest & 0.74 & 21 \\
\hline
sphinx & 0.54 & 19 & xz & 1.09 & 10 \\
\hline
monetDB & 1.32 & 3.4 & cam4 & 1.10 & 5\\ %
\hline
xapian & 1.77 & 1.6 &  cactusBSSN & 1.12 & 7.8 \\
\hline
bc & 0.22 & 48 &  wrf & 1.16 & 4.9  \\ 
\hline
pr & 0.53 & 21 & mcf & 1.28 & 10 \\ 
\hline
cc & 0.67 & 16 & nab & 1.73 & 0.87  \\
\hline
sssp & 0.91 & 10 & perlbench & 1.73 & 0.7 \\
\hline
tc & 1.0 & 15 & leela & 1.87 & 0.18 \\ 
\hline
bfs & 1.24 & 10 & povray & 1.91 & 0.02  \\
\hline
\multicolumn{3}{c|}{} & deepsjeng & 2.25 & 0.34 \\ 
\cline{4-6}
\end{tabular}

\end{footnotesize}
\end{center}
\end{table}


